Know2BIO: A Comprehensive Dual-View Benchmark for Evolving Biomedical Knowledge Graphs

Knowledge graphs (KGs) have emerged as a powerful framework for representing and integrating complex biomedical information. However, assembling KGs from diverse sources remains a significant challenge in several aspects, including entity alignment, scalability, and the need for continuous updates to keep pace with scientific advancements. Moreover, the representative power of KGs is often limited by the scarcity of multi-modal data integration. To overcome these challenges, we propose Know2BIO, a general-purpose heterogeneous KG benchmark for the biomedical domain. Know2BIO integrates data from 30 diverse sources, capturing intricate relationships across 11 biomedical categories. It currently consists of ~219,000 nodes and ~6,200,000 edges. Know2BIO is capable of user-directed automated updating to reflect the latest knowledge in biomedical science. Furthermore, Know2BIO is accompanied by multi-modal data: node features including text descriptions, protein and compound sequences and structures, enabling the utilization of emerging natural language processing methods and multi-modal data integration strategies. We evaluate KG representation models on Know2BIO, demonstrating its effectiveness as a benchmark for KG representation learning in the biomedical field. Data and source code of Know2BIO are available at https://github.com/Yijia-Xiao/Know2BIO/.

==> app/models.tex <==
The KG representation learning models used for experiments can be classified into five categories: translation-based models, bilinear models, neural network models, complex vector models, and hyperbolic space models.

\emph{Translation-based models}, also known as Trans-X models, conceptualize relations as translation operations on the representations of entities. For example, TransE perceives each relation type as a translation operator that moves from the head entity to the tail entity. The principle of this movement can be represented mathematically as $v_h + v_r \approx v_t$. TransE is particularly suited for capturing 1-to-1 relationships, where each head entity is linked to a maximum of 1 tail entity for a given relation type. Later, TransH, TransR, and TransD extended the core idea of translation-based representation.

\emph{Bilinear models} such as DISTMULT represent each relation as a diagonal matrix, facilitating interactions between entity pairs. SimplE is an extension of DISTMULT, allowing for the learning of two dependent embeddings for each entity.

\emph{Neural network models} leverage neural networks (e.g. convolutional neural networks) for knowledge graph embedding. ConvE and ConvKB are prime examples. ConvE employs a convolution layer directly on the 2D reshaping of the embeddings of the head entity and relation. ConvKB applies a convolution layer over embedding triples. Each of these triples is represented as a 3-column matrix, where each column vector represents one element of the triple.

\emph{Complex vector} models use vectors from Complex or Euclidean space to expand their expressive capacity. Notable examples include ComplEx, RotatE, and AttE.

\emph{Hyperbolic space models} take advantage of hyperbolic space’s ability to represent hierarchical structures with minimal distortion. In Euclidean space, distances between points are measured using the Euclidean metric, which assumes a flat space. However, in hyperbolic space, distances are measured using the hyperbolic metric, which takes into account the negative curvature of the space. This property allows hyperbolic space models to capture long-range dependencies more efficiently than Euclidean space models. Models like RefH and AttH enhance the quality of KG embedding by incorporating hyperbolic geometry and attention mechanisms to model complex relational patterns.

